A lipid-structured mathematical model of atherosclerosis with macrophage proliferation

We extend the lipid-structured model for atherosclerotic plaque development of Ford et al. (2019) to account for macrophage proliferation. Proliferation is modelled as a non-local decrease in the lipid structural variable that is similar to the treatment of cell division in size-structured models (e.g. Efendiev et al. (2018)). Steady state analysis indicates that proliferation assists in reducing eventual necrotic core size and acts to spread the lipid load of the macrophage population amongst the cells. The relative contribution of plaque macrophages by proliferation and recruitment from the bloodstream is also examined. The model suggests that a more proliferative plaque differs from an equivalent (same lipid content and cell count) recruitment-dominant plaque only in the way lipid is distributed amongst the macrophages.

==> Template files/sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


